Synthesizing Public Opinions with LLMs: Role Creation, Impacts, and the Future to eDemorcacy

This paper investigates the use of Large Language Models (LLMs) to synthesize public opinion data, addressing challenges in traditional survey methods like declining response rates and non-response bias. We introduce a novel technique: role creation based on knowledge injection, a form of in-context learning that leverages RAG and specified personality profiles from the HEXACO model and demographic information, and uses that for dynamically generated prompts. This method allows LLMs to simulate diverse opinions more accurately than existing prompt engineering approaches. We compare our results with pre-trained models with standard few-shot prompts. Experiments using questions from the Cooperative Election Study (CES) demonstrate that our role-creation approach significantly improves the alignment of LLM-generated opinions with real-world human survey responses, increasing answer adherence. In addition, we discuss challenges, limitations and future research directions.

==> sec/profiler.tex <==
\section{Voter Role Creation}

For our LLMs to encode specific voter preferences into the system, we propose a dynamic voter role creation framework. This allows us to dynamically create a varied number of voter profiles that we can later use to prompt an LLM to produce outputs aligned more with those profiles. On a very high level To dynamically create personal preferences in LLMs, we leverage psychological frameworks such as the HEXACO personality model. This provides a structured way to define and manipulate personal traits.

\subsection{Methods for Creating Personal Preferences}

Our method of injecting these roles is specifically by crafting prompts that explicitly instruct the LLM to embody specific personal traits. 

\subsection{Deriving Role from Attributes} \label{sec:profilederevation}

We present two scalable methods for creating diverse user roles for our experiments, using properties derived from partisan values: Text-to-Role and Role-to-Role. These methods aim to capture the complex connections between online content and the characteristics of individuals who engage with it, particularly within the context of political discourse and the formation of public opinion.

\subsubsection{Text-to-Role Generation}\label{sec:t2p}

This method rests on the principle that an individual's professional background, cultural heritage, and socio-political views significantly shape their online interactions, including how they consume and create content. Therefore, we propose that analyzing a given text can reveal attributes of a hypothetical profile likely to have a particular interaction (e.g., agreement, disagreement, creation, sharing) with that text. Given the virtually limitless and diverse textual data accessible on the Web, this method facilitates the derivation of a wide array of profiles.

